Near-Optimal Resilient Aggregation Rules for Distributed Learning Using 1-Center and 1-Mean Clustering with Outliers

Byzantine machine learning has garnered considerable attention in light of the unpredictable faults that can occur in large-scale distributed learning systems. The key to secure resilience against Byzantine machines in distributed learning is resilient aggregation mechanisms. Although abundant resilient aggregation rules have been proposed, they are designed in ad-hoc manners, imposing extra barriers on comparing, analyzing, and improving the rules across performance criteria. This paper studies near-optimal aggregation rules using clustering in the presence of outliers. Our outlier-robust clustering approach utilizes geometric properties of the update vectors provided by workers. Our analysis show that constant approximations to the 1-center and 1-mean clustering problems with outliers provide near-optimal resilient aggregators for metric-based criteria, which have been proven to be crucial in the homogeneous and heterogeneous cases respectively. In addition, we discuss two contradicting types of attacks under which no single aggregation rule is guaranteed to improve upon the naive average. Based on the discussion, we propose a two-phase resilient aggregation framework. We run experiments for image classification using a non-convex loss function. The proposed algorithms outperform previously known aggregation rules by a large margin with both homogeneous and heterogeneous data distributions among non-faulty workers. Code and appendix are available at https://github.com/jerry907/AAAI24-RASHB.

==> femnist_cnn_niid_pga_0.1.tex <==
\begin{table}[ht]
    \centering
    \caption{Performance comparison under PGA attack on FEMNIST with the nonuniform sampling at an adversarial rate of $0.1$.}
    \label{tab:niid_pga}
    \scalebox{0.75}{
    \begin{tabular}{ccccccccccccccccccccc}
        \toprule
        FedAvg & GM & CClip & CWM & CWTM & Krum & Cent2P & Mean2P \\
        \midrule
        0.01 & 0.00 & 0.43 & 0.12 & 0.04 & 0.19 & 0.87 \cellcolor{lightGreen} & 0.87 \cellcolor{lightGreen}\\
        \bottomrule
    \end{tabular}
    }
\end{table}
